End-to-End Modelling of Earthquake-Induced Polarisation Perturbations in Submarine Optical Fibres

We present an end-to-end model of earthquake-perturbed signal propagation in submarine fibres. Ground displacements are converted to fibre strain via ocean pressure, and injected into a split-step model. Our model shows good qualitative alignment with measurements from the Curie cable during the 2020 Oaxaca earthquake.

==> figures/birefringence.tex <==
\begin{axis}[
    name = Poincare,
    axis lines = center,
    axis equal,
    scale uniformly strategy = units only,
    view/h = 110,
    view/v = 25,
    at = {(0, 0)},
    font = \footnotesize,
    anchor = center,
    width = 5cm,
    height = 5cm,
    axis line style = {gray},
    xmin = -1.3,
    xmax = 1.3,
    ymin = -1.3,
    ymax = 1.3,
    zmin = -1.3,
    zmax = 1.3,
    xtick = \empty,
    ytick = \empty,
    ztick = \empty,
    xlabel = $S_1$,
    ylabel = $S_2$,
    zlabel = $S_3$,
    xlabel style = {gray, xshift = -3pt, yshift = -9pt},
    ylabel style = {gray},
    zlabel style = {gray},
    samples = 31,
    samples y = 1,
    variable = \x,
    domain = 0:360,
    remember picture
]
    % S1, S2 plane
    \addplot3[ForestGreen, densely dotted] ({cos(x)}, {sin(x)}, 0);
    % S1, S3 plane
    \addplot3[BrickRed, densely dotted] ({cos(x)}, 0, {sin(x)});
    % S2, S3 plane
    \addplot3[NavyBlue, densely dotted] (0, {cos(x)}, {sin(x)});

    % % SOP vector
    % \node[inner sep = .5em] (DGD) at ({cos(40) * cos(70)}, {cos(40) * sin(70)}, {sin(40)}) {};
    % % \node[at = (DGD.east), anchor = south west, xshift = -1.4em] {$\vec A_{k-1}(\omega)$};
    % \draw[->, line width = 1pt] (0, 0, 0) -- (DGD.center);

    % rotation axis and major angle
    \addplot3[
        dotted,
        line width = 1.5pt
    ] coordinates {(0, 0, 0) ({cos(25)}, {sin(25)}, 0)};
    \addplot3[
        domain = 0:25,
        samples = 10
    ] ({0.6 * cos(x)}, {0.6 * sin(x)}, 0) node[midway, anchor = north] {$2\theta_k$};

    % % Rotated SOP
    % \node[inner sep = .5em] (DGDRotated) at ({cos(40) * cos(-20)}, {cos(40) * sin(-20)}, {sin(40)}) {};
    % \draw[->, line width = 1pt] (0, 0, 0) -- (DGDRotated.center);
    
    % % birefringence angle
    % \coordinate (RotationPoint) at ({0.5 * cos(40) * (cos(70) + cos(-20))}, {0.5 * cos(40) * (sin(70) + sin(-20))}, 0);
    % \draw[dashed] (DGD.center) -- (RotationPoint) -- (DGDRotated.center);
    % \addplot3[
    %     domain = 50:130,
    %     samples = 20
    % ] ({0.5 * cos(40) * (cos(70) + cos(-20)) + 0.3 * cos(x) * cos(25 + 90)}, {0.5 * cos(40) * (sin(70) + sin(-20)) + 0.3 * cos(x) * sin(25 + 90)}, {0.3 * sin(x)}) node[midway, anchor = south] {$\Delta\beta(\omega)$};

    % Rotation path
    \addplot3[
        -{Latex[length=2mm]},
        % BrickRed,
        % dashed,
        line width = 1.5pt,
        domain = 50:130,
        samples = 20
    ] ({0.5 * cos(40) * (cos(70) + cos(-20)) + 0.84 * cos(x) * cos(25 + 90)}, {0.5 * cos(40) * (sin(70) + sin(-20)) + 0.84 * cos(x) * sin(25 + 90)}, {0.84 * sin(x)}) node[midway, anchor = north, black] {$-2b$};% node[pos = 0, anchor = north west, shift = {(-12pt, 0pt)}] {$\vec S_{k-1}(t')$} node[anchor = east] {$\vec S_k(t')$};
    % \node[anchor = north, yshift = .1em] at ({0.5 * cos(40) * (cos(70) + cos(-20)) + 0.84 * cos(130) * cos(25 + 90)}, {0.5 * cos(40) * (sin(70) + sin(-20)) + 0.84 * cos(130) * sin(25 + 90)}, {0.84 * sin(130)}) {$\vec A_k(\omega)$};
\end{axis}
\node[anchor = north, yshift = -.7em] at (Poincare.north) {Poincar\'e Sphere};


==> figures/fibre.tex <==
\footnotesize

% Draw fibre input
\node[field] (Input) {$\vec A_0(\omega)$};

% Draw fibre steps
\coordinate (Fibre1) at ($(Input.east) + (\nodeDistance + \fibreRadius, 0)$);

\draw[draw = none, fill = \fibreEdgeColour] ($(Fibre1) + (0, \fibreRadius)$) -- ++(\sectionCount\sectionLength, 0) arc (90:-90:\fibreRadius) -- ++(-\sectionCount\sectionLength, 0) arc (-90:-270:\fibreRadius);

\draw (Fibre1) circle (\fibreRadius);

\foreach \index [
    evaluate = \index as \indexPlusOne using int(\index + 1)
] in {1,...,\sectionCount}{
    \coordinate[right = \sectionLength of Fibre\index] (Fibre\indexPlusOne);
    \draw ($(Fibre\indexPlusOne) + (0, \fibreRadius)$) arc (90:-90:\fibreRadius);
    \ifthenelse{\index < \sectionCountMinusOne}{
        \node[field, anchor = south] at ($(Fibre\index)!.5!(Fibre\indexPlusOne) + (0, \fibreRadius + .2em)$) {$k = \index$};
    }{}
    \ifthenelse{\index = \sectionCountMinusOne}{
        \node[field] at ($(Fibre\index)!.5!(Fibre\indexPlusOne) + (\fibreRadius, 0)$) {$\cdots$};
    }{}
    \ifthenelse{\index = \sectionCount}{
        \node[field, anchor = south] at ($(Fibre\index)!.5!(Fibre\indexPlusOne) + (0, \fibreRadius + .2em)$) {$k = K$};
    }
}
\draw ($(Fibre1) + (0, \fibreRadius)$) -- ($(Fibre\sectionCountPlusOne) + (0, \fibreRadius)$);
\draw ($(Fibre1) + (0, -\fibreRadius)$) -- ($(Fibre\sectionCountPlusOne) + (0, -\fibreRadius)$);

% Draw step length
\draw[<->] ($(Fibre1) - (0, \fibreRadius + .35em)$) -- ++(\sectionLength, 0) node[midway, anchor = north] {$\Delta z$};

% Draw fibre output
\node[field, right = \nodeDistance + \fibreRadius of Fibre\sectionCountPlusOne] (Output) {$\vec A_K(\omega)$};

% Draw connections
\draw[arrow] (Input) -- (Fibre1.center);
\draw[arrow] ($(Fibre\sectionCountPlusOne) + (\fibreRadius, 0)$) -- (Output);

==> figures/filter.tex <==
\begin{loglogaxis}[
    font = \footnotesize,
    name = FilterPlot,
    height = 3cm,
    width = 4cm,
    xlabel = {Frequency [\unit{\hertz}]},
    ylabel = {Freq. response},
    ylabel style = {align = center, yshift = -.5em, xshift = -.5em},
    grid,
    xmin = 1e-3, xmax = 1,
]
    \addplot [
        \earthquakeColour,
        thick,
        no markers,
        line width = 1.5pt
    ]
    table [
        col sep = comma,
        x index = 0,
        y index = 1
    ] {figures/pacific_response.csv};
\end{loglogaxis}%

==> figures/map.tex <==
\footnotesize

% \def\longitudeStart{-122}
% \def\longitudeStop{-70}
% \def\latitudeStart{-35}
% \def\latitudeStop{36}
\def\longitudeStart{-142}
\def\longitudeStop{-50}
\def\latitudeStart{-55}
\def\latitudeStop{56}

\pgfmathparse{(\latitudeStop - \latitudeStart) / (\longitudeStop - \longitudeStart)}
\newlength\mapHeight
\setlength\mapHeight{\pgfmathresult\mapWidth}

% Draw background map
\node[anchor = south west, inner sep = 0] {\includegraphics[width = \mapWidth]{figures/map_empty.pdf}};

\begin{scope}[
        x = \mapWidth / (\longitudeStop - \longitudeStart),
        y = \mapHeight / (\latitudeStop - \latitudeStart),
        shift = {(-\longitudeStart, -\latitudeStart)}
    ]    
    % Draw fibre segments and points from submarine cable map
    \edef\oldLongitude{-71.62043502747198}
    \edef\oldLatitude{-33.04554123247811}
    \pgfplotsforeachungrouped \longitude/\latitude in {%
        -72.67487428049728/-31.85146566557725,
        -79.64986933934534/-18.45381377577717,
        -84.14986615150535/-11.503333845984299,
        -85.4998651951533/-6.616650693475355,
        -85.94986487636929/0.568578852526193,
        -87.06475643430802/5.534179292238662,
        -92.69986009460932/9.52441134501949,
        -98.09985626920157/12.615395567393394,
        -104.39985180622544/16.10232559580297,
        -108.44984893716946/18.678647022154717,
        -114.29984479297735/22.469443964829516,
        -118.79984160513736/27.76358852605777,
        -119.6998409675696/31.286738814391754,
        -119.24984128635361/32.8123187832876,
        -118.79984160513764/33.75276987113061,
        -118.41596126184768/33.91992001851462
    }{%
        \draw[fibre, \fibreEdgeColour]
        (\oldLongitude, \oldLatitude) --
        (\longitude, \latitude);
    
        \draw[fibre, draw = none, fill = \fibreVertexColour] (\oldLongitude, \oldLatitude) circle (.5\fibreWidth);%
        
        \edef\oldLongitude{\longitude}
        \edef\oldLatitude{\latitude}
    }
    \draw[fibre, draw = none, fill = \fibreVertexColour] (\oldLongitude, \oldLatitude) circle (.5\fibreWidth);%
    
    % Draw earthquake
    \node[inner sep = \earthquakeWidth / \earthquakeRingCount] (Earthquake) at (-96.07, 16.02) {};
    \draw[earthquake, draw = none] (Earthquake) circle (\earthquakeWidth / \earthquakeRingCount);
    \foreach \ringIndex in {2, ..., \earthquakeRingCount} {
        \draw[earthquake, fill = none] (Earthquake) circle (\earthquakeWidth / \earthquakeRingCount * \ringIndex);
    }
    
    % Draw cities
    % \coordinate (Valparaiso) at (-72.67, -31.85);
    % \node[anchor = west, text = black, rotate = -\mapRotation] at (Valparaiso) {\large{Valparaiso}};

\coordinate (Valparaiso) at (-72.67, -31.85);
\node[anchor = south, text = black, rotate = -\mapRotation, yshift = 6pt, xshift=14pt] (ValparaisoLabel) at (Valparaiso) {\small{\textbf{Valparaiso}}};
\draw[->, thick] (ValparaisoLabel) -- (Valparaiso);

    % \coordinate (LosAngeles) at (-118.42, 33.92);
    % \node[anchor = east, text = black, rotate = -\mapRotation] (LosAngelos) at (LosAngeles) {\large\textbf{Los Angeles}};
\coordinate (LosAngeles) at (-118.42, 33.92);
\node[anchor = south, text = black, rotate = -\mapRotation, yshift = 5.5pt, xshift=-20pt] (LosAngelesLabel) at (LosAngeles) {\small{\textbf{Los Angeles}}};
\draw[->, thick] (LosAngelesLabel) -- (LosAngeles);

    % \coordinate (Oaxaca) at (-96.73, 17.07);
    % \node[anchor = east, text = black, rotate = -\mapRotation] at (Oaxaca) {\large{Oaxaca}};
\coordinate (Oaxaca) at (-96.73, 17.07);
\node[anchor = south, text = black, rotate = -\mapRotation, yshift = 28pt, xshift=-14pt] (OaxacaLabel) at (Oaxaca) {\small{\textbf{Oaxaca}}};
\draw[->, thick] (OaxacaLabel) -- (Oaxaca);
\end{scope}
